Commissioning, Calibration, and Performance of the Cherenkov Telescope on EUSO-SPB2

The detection of astrophysical neutrinos by IceCube in the TeV-PeV energy range motivates the development of instruments for observing these particles at higher energies. Moreover, the detection of very-high-energy (VHE) neutrinos could potentially bring constraints on ultra-high energy cosmic rays (UHECRs) source models. Tau neutrinos skimming the Earth under a shallow angle can be detected through the decay of a tau resulting in an extensive air shower (EAS) in the atmosphere. The EAS can be detected by capturing some of the optical Cherenkov signal originating from the EAS particles. To assess the feasibility of the Earth-skimming technique from high altitudes, we developed a Cherenkov telescope which was deployed on the Extreme Universe Space Observatory Super Pressure Balloon 2 (EUSO-SPB2) from Wanaka, NZ, on May $13^{th}$. It is a precursor for the Probe of Extreme Multi-Messenger Astrophysics. The 1m diameter Cherenkov telescope for EUSO-SPB2 had a focal plane comprised of 512 silicon photomultipliers (SiPMs) covering a 6.4 x 12.8 square degree field of view coupled to a 100 MS/s readout based on the GET switch capacitor ring sampler. We discuss the calibration and commissioning of the telescope and its in-flight performance.

==> JEM-EUSO_Authors_July2023.tex <==
\begin{sloppypar}
{\small \noindent
S.~Abe$^{fq}$, 
J.H.~Adams Jr.$^{pd}$, 
D.~Allard$^{cb}$,
P.~Alldredge$^{pd}$,
L.~Anchordoqui$^{pe}$,
A.~Anzalone$^{eh,ed}$, 
E.~Arnone$^{ek,el}$,
M.~Bagheri$^{ph}$,
B.~Baret$^{cb}$,
D.~Barghini$^{el,ek}$,
M.~Battisti$^{ek,el,cb}$,
R.~Bellotti$^{ea,eb}$, 
A.A.~Belov$^{kb}$, 
M.~Bertaina$^{ek,el}$,
P.F.~Bertone$^{pf}$,
M.~Bianciotto$^{ek,el}$,
P.L.~Biermann$^{db}$,
F.~Bisconti$^{ei}$, 
C.~Blaksley$^{ft}$, 
S.~Blin-Bondil$^{cb}$, 
K.~Bolmgren$^{na}$,
S.~Briz$^{pb}$,
J.~Burton$^{pd}$,
F.~Cafagna$^{ea.eb}$, 
G.~Cambi\'e$^{ei,ej}$,
D.~Campana$^{ef}$, 
F.~Capel$^{de}$, 
R.~Caruso$^{ec,ed}$, 
M.~Casolino$^{ft,ei, ej}$,
C.~Cassardo$^{ek,el}$, 
A.~Castellina$^{ek,em}$,
K.~\v{C}ern\'{y}$^{bb}$,  
M.J.~Christl$^{pf}$, 
R.~Colalillo$^{ef,eg}$,
L.~Conti$^{en,ei}$, 
G.~Cotto$^{ek,el}$, 
H.J.~Crawford$^{pa}$, 
R.~Cremonini$^{el}$,
A.~Creusot$^{cb}$, 
A.~de Castro G\'onzalez$^{pb}$,  
C.~de la Taille$^{ca}$, 
R.~Diesing$^{pb}$,
P.~Dinaucourt$^{ca}$,
A.~Di Nola$^{eg}$,
A.~Ebersoldt$^{db}$,
T.~Ebisuzaki$^{ft}$,
J.~Eser$^{pb}$,
F.~Fenu$^{eo}$, 
S.~Ferrarese$^{ek,el}$,
G.~Filippatos$^{pc}$, 
W.W.~Finch$^{pc}$,
F. Flaminio$^{eg}$,
C.~Fornaro$^{en,ei}$,
D.~Fuhne$^{pc}$,
C.~Fuglesang$^{na}$, 
M.~Fukushima$^{fe}$, 
S.~Gadamsetty$^{ph}$,
D.~Gardiol$^{ek,em}$,
G.K.~Garipov$^{kb}$, 
E.~Gazda$^{ph}$, 
A.~Golzio$^{ek,el}$,
F.~Guarino$^{ef,eg}$, 
C.~Gu\'epin$^{pb}$,
A.~Haungs$^{db}$,
T.~Heibges$^{pc}$,,
F.~Isgr\`o$^{ef,eg}$, 
E.G.~Judd$^{pa}$, 
F.~Kajino$^{ff}$, 
I.~Kaneko$^{ft}$, 
M.~Kleifges$^{db}$,
P.A.~Klimov$^{kb}$,
I.~Kreykenbohm$^{da}$, 
J.F.~Krizmanic$^{pj}$, 
V.~Kungel$^{pc}$,  
E.~Kuznetsov$^{pd}$, 
F.~L\'opez~Mart\'inez$^{pb}$, 
D.~Mand\'{a}t$^{bc}$,
M.~Manfrin$^{ek,el}$,
A. Marcelli$^{ej}$,
L.~Marcelli$^{ei}$, 
W.~Marsza{\l}$^{ia}$, 
J.N.~Matthews$^{pg}$, 
A.~Menshikov$^{db}$,
M.~Mese$^{ef,eg}$, 
S.S.~Meyer$^{pb}$,
J.~Mimouni$^{ad}$, 
H.~Miyamoto$^{ek,el}$, 
Y.~Mizumoto$^{fi}$,
A.~Monaco$^{ea,eb}$, 
S.~Nagataki$^{ft}$, 
J.~M.~Nachtman$^{pi}$,
D.~Naumov$^{ka}$,
A.~Neronov$^{cb}$,  
T.~Nonaka$^{fe}$, 
T.~Ogawa$^{ft}$, 
S.~Ogio$^{ft}$, 
H.~Ohmori$^{ft}$, 
A.V.~Olinto$^{pb}$,
Y.~Onel$^{pi}$,
G.~Osteria$^{ef}$,  
A.N.~Otte$^{ph}$,  
A.~Pagliaro$^{eh,ed}$,  
B.~Panico$^{ef, eg}$,  
E.~Parizot$^{cb, cd}$, 
I.H.~Park$^{gb}$, 
T.~Paul$^{pe}$,
M.~Pech$^{bc}$, 
F.~Perfetto$^{ef}$,  
P.~Picozza$^{ei,ej}$, 
L.W.~Piotrowski$^{ib}$,
Z.~Plebaniak$^{ei, ej}$, 
J.~Posligua$^{pi}$,
M.~Potts$^{ph}$,
R.~Prevete$^{ef,eg}$,
G.~Pr\'ev\^ot$^{cb}$,
M.~Przybylak$^{ia}$, 
E.~Reali$^{ei, ej}$,
P.~Reardon$^{pd}$, 
M.H.~Reno$^{pi}$, 
M.~Ricci$^{ee}$, 
O.F.~Romero~Matamala$^{ph}$, 
G.~Romoli$^{ei, ej}$,
H.~Sagawa$^{fe}$, 
N.~Sakaki$^{ft}$, 
A.~Santangelo$^{dd}$, 
O.A.~Saprykin$^{kc}$,
F.~Sarazin$^{pc}$,
M.~Sato$^{fo}$, 
H.~Schieler$^{db}$,
P.~Schov\'{a}nek$^{bc}$,
V.~Scotti$^{ef,eg}$,
S.~Selmane$^{cb}$
S.A.~Sharakin$^{kb}$,
K.~Shinozaki$^{ia}$, 
S.~Stepanoff$^{ph}$,
J.F.~Soriano$^{pe}$,
J.~Szabelski$^{ia}$,
N.~Tajima$^{ft}$, 
T.~Tajima$^{ft, pn}$,
Y.~Takahashi$^{fo}$, 
M.~Takeda$^{fe}$, 
Y.~Takizawa$^{ft}$, 
C.~Tenzer$^{dd}$,
S.B.~Thomas$^{pg}$, 
L.G.~Tkachev$^{ka}$,
T.~Tomida$^{fh}$, 
S.~Toscano$^{ob}$,  
M.~Tra\"{i}che$^{aa}$,  
D.~Trofimov$^{cb,kb}$,
K.~Tsuno$^{ft}$,  
P.~Vallania$^{ek,em}$,
L.~Valore$^{ef,eg}$,
T.~M.~Venters$^{pj}$,
C.~Vigorito$^{ek,el}$, 
M.~Vrabel$^{ia}$, 
S.~Wada$^{ft}$,  
J.~Watts~Jr.$^{pd}$, 
A.~Weindl$^{db}$,
L.~Wiencke$^{pc}$, 
J.~Wilms$^{da}$,
D.~Winn$^{pm}$,
H.~Wistrand$^{pc}$,
I.V.~Yashin$^{kb}$, 
R.~Young$^{pf}$,
M.Yu.~Zotov$^{kb}$.
}
\end{sloppypar}
\vspace*{.3cm}

%%\newpage
{ \footnotesize
\noindent
% Algeria - 2 institutes
$^{aa}$ Centre for Development of Advanced Technologies (CDTA), Algiers, Algeria \\
$^{ad}$ Lab. of Math. and Sub-Atomic Phys. (LPMPS), Univ. Constantine I, Constantine, Algeria \\
% Czech Republic - 2 institutes
$^{bb}$ Joint Laboratory of Optics, Faculty of Science, Palack\'{y} University, Olomouc, Czech Republic\\
$^{bc}$ Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic\\
% France - 3 institutes  
$^{ca}$ Omega, Ecole Polytechnique, CNRS/IN2P3, Palaiseau, France\\
$^{cb}$ Universit\'e de Paris, CNRS, AstroParticule et Cosmologie, F-75013 Paris, France\\
$^{cd}$ Institut universitaire de France (IUF)\\
% Germany - 4 institutes
$^{da}$ ECAP, University of Erlangen-Nuremberg, Germany\\
$^{db}$ Karlsruhe Institute of Technology (KIT), Germany\\
$^{dd}$ Institute for Astronomy and Astrophysics, Kepler Center, University of T\"ubingen, Germany\\
$^{de}$ Max Planck Institute for Physics, Munich, Germany\\
% Italy - 15 institutes  
$^{ea}$ Istituto Nazionale di Fisica Nucleare - Sezione di Bari, Italy\\
$^{eb}$ Universita' degli Studi di Bari Aldo Moro and INFN - Sezione di Bari, Italy\\
$^{ec}$ Dipartimento di Fisica e Astronomia "Ettore Majorana", Universita' di Catania, Italy\\
$^{ed}$ Istituto Nazionale di Fisica Nucleare - Sezione di Catania, Italy\\
$^{ee}$ Istituto Nazionale di Fisica Nucleare - Laboratori Nazionali di Frascati, Italy\\
$^{ef}$ Istituto Nazionale di Fisica Nucleare - Sezione di Napoli, Italy\\
$^{eg}$ Universita' di Napoli Federico II - Dipartimento di Fisica "Ettore Pancini", Italy\\
$^{eh}$ INAF - Istituto di Astrofisica Spaziale e Fisica Cosmica di Palermo, Italy\\
$^{ei}$ Istituto Nazionale di Fisica Nucleare - Sezione di Roma Tor Vergata, Italy\\
$^{ej}$ Universita' di Roma Tor Vergata - Dipartimento di Fisica, Roma, Italy\\
$^{ek}$ Istituto Nazionale di Fisica Nucleare - Sezione di Torino, Italy\\
$^{el}$ Dipartimento di Fisica, Universita' di Torino, Italy\\
$^{em}$ Osservatorio Astrofisico di Torino, Istituto Nazionale di Astrofisica, Italy\\
$^{en}$ Uninettuno University, Rome, Italy\\
$^{eo}$ Agenzia Spaziale Italiana, Via del Politecnico, 00133, Roma, Italy\\
% Japan - 7 institutes 
$^{fe}$ Institute for Cosmic Ray Research, University of Tokyo, Kashiwa, Japan\\ 
$^{ff}$ Konan University, Kobe, Japan\\ 
$^{fh}$ Shinshu University, Nagano, Japan \\
$^{fi}$ National Astronomical Observatory, Mitaka, Japan\\ 
$^{fo}$ Hokkaido University, Sapporo, Japan \\ 
$^{fq}$ Nihon University Chiyoda, Tokyo, Japan\\ 
$^{ft}$ RIKEN, Wako, Japan\\
% Korea - 1 institute
$^{gb}$ Sungkyunkwan University, Seoul, Republic of Korea\\
% Poland - 2 institutes
$^{ia}$ National Centre for Nuclear Research, Otwock, Poland\\
$^{ib}$ Faculty of Physics, University of Warsaw, Poland\\
% Russia - 3 institutes 
$^{ka}$ Joint Institute for Nuclear Research, Dubna, Russia\\
$^{kb}$ Skobeltsyn Institute of Nuclear Physics, Lomonosov Moscow State University, Russia\\
$^{kc}$ Space Regatta Consortium, Korolev, Russia\\
% Sweden - 1 institute 
$^{na}$ KTH Royal Institute of Technology, Stockholm, Sweden\\
% Switzerland - 1 institute 
$^{ob}$ ISDC Data Centre for Astrophysics, Versoix, Switzerland\\
% USA - 12 institutes 
$^{pa}$ Space Science Laboratory, University of California, Berkeley, CA, USA\\
$^{pb}$ University of Chicago, IL, USA\\
$^{pc}$ Colorado School of Mines, Golden, CO, USA\\
$^{pd}$ University of Alabama in Huntsville, Huntsville, AL; USA\\
$^{pe}$ Lehman College, City University of New York (CUNY), NY, USA\\
$^{pf}$ NASA Marshall Space Flight Center, Huntsville, AL, USA\\
$^{pg}$ University of Utah, Salt Lake City, UT, USA\\
$^{ph}$ Georgia Institute of Technology, USA\\
$^{pi}$ University of Iowa, Iowa City, IA, USA\\
$^{pj}$ NASA Goddard Space Flight Center, Greenbelt, MD, USA\\
$^{pm}$ Fairfield University, Fairfield, CT, USA\\
$^{pn}$ Department of Physics and Astronomy, University of California, Irvine \\
}

